CounterNet: End-to-End Training of Prediction Aware Counterfactual Explanations

This work presents CounterNet, a novel end-to-end learning framework which integrates Machine Learning (ML) model training and the generation of corresponding counterfactual (CF) explanations into a single end-to-end pipeline. Counterfactual explanations offer a contrastive case, i.e., they attempt to find the smallest modification to the feature values of an instance that changes the prediction of the ML model on that instance to a predefined output. Prior techniques for generating CF explanations suffer from two major limitations: (i) all of them are post-hoc methods designed for use with proprietary ML models -- as a result, their procedure for generating CF explanations is uninformed by the training of the ML model, which leads to misalignment between model predictions and explanations; and (ii) most of them rely on solving separate time-intensive optimization problems to find CF explanations for each input data point (which negatively impacts their runtime). This work makes a novel departure from the prevalent post-hoc paradigm (of generating CF explanations) by presenting CounterNet, an end-to-end learning framework which integrates predictive model training and the generation of counterfactual (CF) explanations into a single pipeline. Unlike post-hoc methods, CounterNet enables the optimization of the CF explanation generation only once together with the predictive model. We adopt a block-wise coordinate descent procedure which helps in effectively training CounterNet's network. Our extensive experiments on multiple real-world datasets show that CounterNet generates high-quality predictions, and consistently achieves 100% CF validity and low proximity scores (thereby achieving a well-balanced cost-invalidity trade-off) for any new input instance, and runs 3X faster than existing state-of-the-art baselines.

==> sections/06_statement.tex <==
\textbf{Ethics Statement.}
Although CounterNet is suitable for real-time deployment given its superior performance in its highly aligned CF explanations and speed, one must be aware of the possible negative impacts of its CF explanations to human end-users. It is important to ensure that generated CF examples do not amplify or provide support to the narratives resulting from pre-existing race-based and gender-based societal inequities (among others).
As we stated in Section~\ref{sec:conclusion}, one short-term workaround is to have humans in the loop. We can provide CounterNet’s explanations as a decision-aid to a well-trained human official, who is in charge of communicating the decisions of ML models to human end-users in a respectful and humane manner. In the long-run, further qualitative and quantitative studies are needed to understand the social impacts of CounterNet.

\textbf{Reproducibility Statement.}
To aid the reproducibility of this work, we provide the code in the supplement material, and will make the code public once it is accepted. We also provide the dataset used for evaluating this paper in this anonymous repository. In addition, we outline the choices of hyperparameters in Appendix~\ref{sec:app-cfnet-detail}. A detailed description of our experimental implementation can be found in Appendix~\ref{sec:app-implementation}. For theoretical analysis of our novel block-wise coordinate descent procedure, we provide complete proof in Appendix~\ref{sec:app-proof}. 

% It is important that the work published in ICLR is reproducible. Authors are strongly encouraged to include a paragraph-long Reproducibility Statement at the end of the main text (before references) to discuss the efforts that have been made to ensure reproducibility. This paragraph should not itself describe details needed for reproducing the results, but rather reference the parts of the main paper, appendix, and supplemental materials that will help with reproducibility. For example, for novel models or algorithms, a link to a anonymous downloadable source code can be submitted as supplementary materials; for theoretical results, clear explanations of any assumptions and a complete proof of the claims can be included in the appendix; for any datasets used in the experiments, a complete description of the data processing steps can be provided in the supplementary materials. Each of the above are examples of things that can be referenced in the reproducibility statement. This optional reproducibility statement will not count toward the page limit, but should not be more than 1 page.


